Precise asymptotics for Fisher-KPP fronts

We consider the one-dimensional Fisher-KPP equation with step-like initial data. Nolen, Roquejoffre, and Ryzhik showed that the solution $u$ converges at long time to a traveling wave $\phi$ at a position $\tilde \sigma(t) = 2t - (3/2)\log t + \alpha_0- 3\sqrt{\pi}/\sqrt{t}$, with error $O(t^{\gamma-1})$ for any $\gamma>0$. With their methods, we find a refined shift $\sigma(t) = \tilde \sigma(t) + \mu_* (\log t)/t + \alpha_1/t$ such that in the frame moving with $\sigma$, the solution $u$ satisfies $u(t,x) = \phi (x) + \psi(x)/t + O(t^{\gamma-3/2})$ for a certain profile $\psi$ independent of initial data. The coefficient $\alpha_1$ depends on initial data, but $\mu_* = 9(5-6\log 2)/8$ is universal, and agrees with a finding of Berestycki, Brunet, and Derrida in a closely-related problem. Furthermore, we predict the asymptotic forms of $\sigma$ and $u$ to arbitrarily high order.

==> colemacros.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Ham}{\mathbb{H}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\Om}{\Omega}
\newcommand{\bd}{\partial}
\newcommand{\h}[1]{\hat{#1}}
\newcommand{\s}[1]{\mathscr{#1}}
\newcommand{\m}[1]{\mathcal{#1}}
\newcommand{\f}[1]{\mathfrak{#1}}
\newcommand{\del}{\nabla}
\newcommand{\der}[2]{\frac{d #1}{d #2}}
\newcommand{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\abs}[1]{\left |#1 \right|}
\newcommand{\norm}[1]{\left \|#1 \right\|}
\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\ti}[1]{\tilde{#1}}
\renewcommand{\bar}[1]{\overline{#1}}
\newcommand{\ubar}[1]{\underline{#1}}
\newcommand{\tbf}[1]{\textbf{#1}}
\newcommand{\id}[1]{\op{id}_{#1}}
\renewcommand{\Re}{\op{Re}}
\renewcommand{\Im}{\op{Im}}
\newcommand{\Ker}{\op{ker}}
\newcommand{\Span}{\op{span}}
\newcommand{\supp}{\op{supp}}
\newcommand{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand{\arccot}{\op{arccot}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand{\MLoc}{\m M_{c,\text{loc}}}
\newcommand{\BM}{Brownian motion}
\newcommand{\nab}{\nabla}
\newcommand{\trdeg}{\op{tr\,deg}}
\newcommand{\gr}{\op{gr}}
\newcommand{\rees}{\op{Rees}}
\newcommand{\Spec}{\op{Spec}}
\renewcommand{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand{\div}{\op{div}}
\newcommand{\power}[1]{{#1}[\![X]\!]}
\newcommand{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\newcommand{\mr}{\mathring}
\newcommand\smallO{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}% \displaystyle
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}% \textstyle
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}% \scriptstyle
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }
